Models of Computational Profiles to Study the Likelihood of DNN Metamorphic Test Cases

Neural network test cases are meant to exercise different reasoning paths in an architecture and used to validate the prediction outcomes. In this paper, we introduce "computational profiles" as vectors of neuron activation levels. We investigate the distribution of computational profile likelihood of metamorphic test cases with respect to the likelihood distributions of training, test and error control cases. We estimate the non-parametric probability densities of neuron activation levels for each distinct output class. Probabilities are inferred using training cases only, without any additional knowledge about metamorphic test cases. Experiments are performed by training a network on the MNIST Fashion library of images and comparing prediction likelihoods with those obtained from error control-data and from metamorphic test cases. Experimental results show that the distributions of computational profile likelihood for training and test cases are somehow similar, while the distribution of the random-noise control-data is always remarkably lower than the observed one for the training and testing sets. In contrast, metamorphic test cases show a prediction likelihood that lies in an extended range with respect to training, tests, and random noise. Moreover, the presented approach allows the independent assessment of different training classes and experiments to show that some of the classes are more sensitive to misclassifying metamorphic test cases than other classes. In conclusion, metamorphic test cases represent very aggressive tests for neural network architectures. Furthermore, since metamorphic test cases force a network to misclassify those inputs whose likelihood is similar to that of training cases, they could also be considered as adversarial attacks that evade defenses based on computational profile likelihood evaluation.

==> experiments.tex <==
\section{Experiments \& Setup}

The experiments in this paper take four image sets into account: train, test, random, and adversarial. To describe the experiments that were performed for this paper and their setup, we will briefly cover the different image sets and the methods with which we dealt with their results. 

\subsection{Train and Test Images}
For the first two image sets, we decided to use the MNIST Fashion library of 70000 images, and split them into 60000 training images and 10000 testing images. Once the deep neural network was trained on the training images using Tensorflow, we began to pass each of them through the network to export and save the corresponding activation values from the last layer in the network. The same was then done with the test images. These two image sets allow us to analyze the activation levels of standard images that the network is familiar with. 
  
We then computed values for statistical parameters such as average, linear variation, and standard deviation for each transition based on the correctly predicted training data. It is important to note that these values were computed per class, and that for each transition, only the correctly predicted images of that particular class were considered in the calculation.

\subsection{Random Images}
On the other side of the spectrum, to analyze how the network reacts on images it is completely unfamiliar with and the effect this may have on their activations, 60000 images of the same size were generated with a script by choosing completely random values for each pixel. Similarly to the previous sets, these images were then passed through the network to obtain the activation values.

\subsection{Rotated Images}
This last image set allows to analyze the activation values of images that the network believes that it recognized, but that have in fact been perturbed. Starting from the same 60000 training images, we perform affine transformations repeatedly until the point that the image prediction goes from correct to incorrect. In the case of this article, we study the effect of rotation on the images.
